KiDS+2dFLenS+GAMA: Testing the cosmological model with the $E_{\rm G}$ statistic

We present a new measurement of $E_{\rm G}$, which combines measurements of weak gravitational lensing, real-space galaxy clustering and redshift space distortions. This statistic was proposed as a consistency test of General Relativity (GR) that is insensitive to linear, deterministic galaxy bias and the matter clustering amplitude. We combine deep imaging data from KiDS with overlapping spectroscopy from 2dFLenS, BOSS DR12 and GAMA and find $E_{\rm G}(\overline{z}=0.267)=0.43 \pm 0.13$ (GAMA), $E_{\rm G}(\overline{z}=0.305)=0.27 \pm 0.08$ (LOWZ+2dFLOZ) and $E_{\rm G}(\overline{z}=0.554)=0.26 \pm 0.07$ (CMASS+2dFHIZ). We demonstrate that the existing tension in the value of the matter density parameter hinders the robustness of this statistic as solely a test of GR. We find that our $E_{\rm G}$ measurements, as well as existing ones in the literature, favour a lower matter density cosmology than the Cosmic Microwave Background. For a flat $\Lambda$CDM Universe and assuming GR, we find $\Omega_{\rm m}(z=0)=0.25\pm0.03$. With this paper we publicly release the 2dFLenS dataset at: \url{http://2dflens.swin.edu.au}.

==> dataandsims.tex <==
\subsection{Kilo Degree Survey (KiDS)} 
\begin{table*}
\caption{ \label{tab:spec} For each spectroscpoic survey used in the analysis, this Table quotes the full area used for the clustering analysis, $A_{\rm full}$, the overlapping area $A_{\rm eff}$ with the KiDS imaging and the number of lenses in the overlap region of each sample that were used in the lensing analyses. Also quoted are the mean redshift of the spectroscopic sample and the RSD measurements of the $\beta$ parameter, taken from \citet{Blake/etal:2016} for 2dFLenS, Singh et al. (in prep.) for the BOSS samples and \citet{Blake2013} for the analysis with GAMA. } 
\begin{center}
\begin{tabular}{lcccccc}
  %\hline
 %{ p{0.2cm}|p{2.5cm}|p{1.0cm}|p{2.0cm}|p{2.0cm}  }
 %\multicolumn{4}{|c|}{xyz} \\
 \hline
Spec. sample & $A_{\rm full}$  (deg$^2$) & $A_{\rm eff}$ (deg$^2$) & $N_{\rm lenses}$ & $\overline{z}$ & $\beta$ \\
 \hline
GAMA & 180 & 144 & 33682 & 0.267 & 0.60 $\pm$ 0.09 \\ %\cline{2-5}
LOWZ & 8337 & 125 & 5656 & 0.309 & 0.41 $\pm$ 0.03 \\
CMASS & 9376 & 222 & 21341 & 0.548 & 0.34 $\pm$ 0.02 \\
2dFLOZ & 731 & 122 & 3014 & 0.300 & 0.49 $\pm$ 0.15 \\ 
2dFHIZ & 731 & 122 & 4662 & 0.560 & 0.26 $\pm$ 0.09 \\ %\cline{2-5}
 \hline
\end{tabular}
\end{center}
\end{table*}

The Kilo-Degree Survey (KiDS) is a large-scale, tomographic, weak-lensing imaging survey \citep{Kuijken/etal:2015} using the wide-field OmegaCAM at the VLT Survey Telescope at ESO Paranal Observatory.  It will span \SI{1350}{\square\degree} on completion, in two patches of the sky with the $ugri$ optical filters, as well as 5 infrared bands from the overlapping VISTA Kilo-degree Infrared Galaxy (VIKING) survey \citep{Edge2013}, yielding the only well-matched wide and deep optical and infrared survey to date. The VLT Survey Telescope is optimally designed for lensing with high-quality optics and the seeing conditions, in the detection $r$-band filter are better than $0.9\arcsec$. 

The fiducial KiDS lensing dataset which is used in this analysis, `KiDS-450', is detailed in \citet{Hildebrandt/etal:2017} with the public data release described in \cite{deJong2017}. This dataset has an effective number density of $n_{\rm eff}=8.5$ galaxies arcmin$^{-2}$ with an effective, unmasked area of \SI{360}{\square\degree}, with its footprint shown in Figure~\ref{fig:map}. Galaxy shapes were measured from the $r$-band data using a self-calibrating version of \textit{lens}fit \citep{miller/etal:2013, fenech-conti/etal:2016} and assigned a lensing weight, $w_{\rm s}$ based on the quality of that galaxy's shape measurement. Utilising a large suite of image simulations, the multiplicative shear bias was deemed to be at the percent level for the entire KiDS ensemble and is accounted for during our cross-correlation measurement. 

The redshift distribution for KiDS galaxies was determined via four different approaches, which were shown to produce consistent results in a cosmic shear analysis \citep{Hildebrandt/etal:2017}. The preferred method that we adopt for this analysis is the `weighted direct calibration' (DIR) method, which exploits an overlap with deep spectroscopic fields. Following the work of \citet{Lima2008}, the spectroscopic galaxies are re-weighted such that any incompleteness in their spectroscopic selection functions is removed. A sample of KiDS galaxies is selected using their associated $z_{\rm B}$ value, estimated from the four-band photometry as the peak of the redshift posterior put out by the Bayesian photometric redshift BPZ code \citep{Benitez2000}. The true redshift distribution for the KiDS sample is determined by matching these to the re-weighted spectroscopic catalogue. 
The resulting redshift distribution is well-calibrated in the range $0.1 < z_{\rm B} \leq 0.9$.

KiDS has full spectroscopic overlap with the Baryon Oscillation Spectroscopic Survey (BOSS) and the Galaxy And Mass Assembly (GAMA) survey in its Northern field and the 2-degree Field Lensing Survey (2dFLenS) in the South. The footprints of the different datasets used in this analysis are shown in Figure~\ref{fig:map} and the effective overlapping areas are quoted in Table~\ref{tab:spec}. 

\subsection{Spectroscopic overlap surveys} 
BOSS is a spectroscopic follow-up of the SDSS imaging survey, which used the Sloan Telescope to obtain redshifts for over a million galaxies spanning \SI{10000}{\square\degree}. BOSS used colour and magnitude cuts to select two classes of galaxies: the `LOWZ' sample, which contains Luminous Red Galaxies (LRGs) at $z_{\rm l} < 0.43$, and the `CMASS' sample, which is designed to be approximately stellar-mass limited for $z_{\rm l} > 0.43$.  We used the data catalogues provided by the SDSS 12th Data Release (DR12); full details of these catalogues are given by \cite{Alam/etal:2015}.  Following standard practice, we select objects from the LOWZ and CMASS datasets with $0.15 < z_{\rm l}  < 0.43$ and $0.43 < z_{\rm l}  < 0.7$, respectively, to create homogeneous galaxy samples. In order to correct for the effects of redshift failures, fibre collisions and other known systematics affecting the angular completeness, we use the completeness weights assigned to the BOSS galaxies \citep{Ross2016}, denoted as $w_{\rm l}$. These are computed as a combination of the systematic weights that calibrate the target density as a function of stellar density and seeing, $w_{\rm systot}$, the no-redshift weights, which upweight the galaxy if its nearest neighbour's redshift could not be determined from the spectrum, $w_{\rm noz}$, and the close-pair fibre collision weights $w_{\rm cp}$, as,
\be
w_{\rm l}=w_{\rm systot}(w_{\rm noz} + w_{\rm cp} - 1) \, .
\ee
The RSD parameters, $\beta$ for LOWZ and CMASS are quoted in Table~\ref{tab:spec} and were drawn from Singh et al. (in prep.), who follow the method described in \citet{Alam2015}. 

2dFLenS is a spectroscopic survey conducted by the Anglo-Australian Telescope with the AAOmega spectrograph, spanning an area of \SI{731}{\square\degree} \citep{Blake/etal:2016}. It is principally located in the KiDS regions, in order to expand the overlap area between galaxy redshift samples and gravitational lensing imaging surveys.  The 2dFLenS spectroscopic dataset contains two main target classes: $\sim$\SI{40000} Luminous Red Galaxies (LRGs) across a range of redshifts $z_{\rm l}< 0.9$, selected by BOSS-inspired colour cuts \citep{Dawson/etal:2013}, as well as a magnitude-limited sample of $\sim$\SI{30000} objects in the range $17<r<19.5$, to assist with direct photometric calibration \citep{wolf/etal:2017, bilicki2017}.  In our study we analyse the 2dFLenS LRG sample, selecting redshift ranges $0.15<z_{\rm l}<0.43$ for `2dFLOZ' and $0.43<z_{\rm l}<0.7$ for `2dFHIZ', mirroring the selection of the BOSS sample.  We refer the reader to \cite{Blake/etal:2016} for a full description of the construction of the 2dFLenS selection function and random catalogues. The RSD parameter was determined by \citep{Blake/etal:2016} from a fit to the multipole power spectra and was found to be $\beta=0.49 \pm 0.15$ and $\beta=0.26 \pm 0.09$ in the low- and high-redshift LRG samples, respectively.

GAMA is a spectroscopic survey carried out on the Anglo-Australian Telescope with the AAOmega spectrograph. We use the GAMA galaxies from three equatorial regions, G9, G12 and G15 from the 3rd GAMA data release \citep{Liske2015}. These equatorial regions encompass roughly \SI{180}{\square\degree}, containing $\sim$\SI{180000} galaxies with sufficient quality redshifts. The magnitude-limited sample is essentially complete down to a magnitude of $r$ = 19.8. For our galaxy-galaxy lensing and clustering measurements, we use all GAMA galaxies in the three equatorial regions in the redshift range $0.15<z_{\rm l}<0.51$. As GAMA is essentially complete, the sample is equally weighted, such that $w_{\rm l}=1$ for all galaxies. We constructed random catalogues using the GAMA angular selection masks combined with an empirical smooth fit to the observed galaxy redshift distribution \citep{Blake2013}. We use the value for the RSD parameter from \citet{Blake2013} as $\beta=0.60 \pm 0.09$, which, we note encompasses a slightly different redshift region of $0.25< z_{\rm l} <0.5$. 


\subsection{Mocks}
We compute the full covariance between the different scales of the galaxy-galaxy lensing measurement using a large suite of $N$-body simulations, built from the Scinet Light Cone Simulations \citep[][SLICS]{HDvW2015} and tailored for weak lensing surveys. These consist of 600 independent dark matter only simulations, in each of which $1536^3$ particles are evolved within a cube of $505 h^{-1} \rm{Mpc}$ on a side and projected on 18 redshift mass planes between $0<z<3$. Light cones are propagated on these planes on $7745^3$ pixel grids and turned into shear maps via ray-tracing, with an opening angle of \SI{100}{\square\degree}. The cosmology is set to $\rm{WMAP9 + BAO + SN}$ \citep{Dunkley}, that is $\Omega_{\rm m}=0.2905$, $\Omega_{\Lambda}=0.7095$, $\Omega_{\rm b}=0.0473$, $h=0.6898$, $n_{\rm s}=0.969$ and $\sigma_8=0.826$.  These mocks are fully described by \citet{HDvW2015} and a previous version with a smaller opening angle of \SI{60}{\square\degree} was used in the KiDS analyses of \citet{Hildebrandt/etal:2017} and \citet{Joudaki2017}. 

Source galaxies are randomly inserted in the mocks, with a true redshift satisfying the KiDS DIR redshift distribution and a mock photometric redshift, $z_{\rm B}$, enabling the selection of source galaxies behind lenses. The source number density is defined to reflect the effective number density of the KiDS data. The gravitational shears are an interpolation of the simulated shear maps at the galaxy positions, while the distribution of intrinsic ellipticity matches a Gaussian with a width of  0.29 per component, closely matching the measured KiDS intrinsic ellipticity dispersion \citep{Amon2017, Hildebrandt/etal:2017}. 

To simulate a foreground galaxy sample, we populate the dark matter haloes extracted from the $N$-body simulations with galaxies, following a halo occupation distribution approach (HOD) that is tailored for each galaxy survey. The details of their construction and their ability to reproduce the clustering and lensing signals with the KiDS and spectroscopic foreground galaxy samples are described in Harnois-D\'eraps et al. (in prep). Here we summarise the strategy. Dark matter haloes are assigned a number of central and satellite galaxies based on their mass and on the HOD prescription. Centrals are placed at the halo centre and satellites are scattered around it following a spherically-symmetric NFW profile, with the number of satellites scaling with the mass of the halo. On average, about 9\% of all mock CMASS and LOWZ galaxies are satellites, a fraction that closely matches that from the BOSS data. The satellite fraction in the GAMA mocks is closer to 15\%. 

The CMASS and LOWZ HODs are inspired by the prescription of \citet{Alam2016} while the GAMA mocks follow the strategy of \citet{Smith2017}. In all three cases, we adjust the value of some of the best-fit parameters in order to enhance the agreement in clustering between mocks and data, while also closely matching the number density and the redshift distribution of the spectroscopic surveys. In contrast to the CMASS and LOWZ mocks, the GAMA mocks are constructed from a conditional luminosity function and galaxies are assigned an apparent magnitude such that we can reproduce the magnitude distribution of the GAMA data. For 2dFLenS, the LOWZ and CMASS mocks were subsampled to match the sparser 2dFLOZ and 2dFHIZ samples. 




%The mean redshift of the mocks is within 3.8\% of the data for LOWZ, 1.3\% for CMASS, 2.5\% for GAMA. The effective number density is 11\% lower than the data for LOWZ (cannot up-sample unfortunately), 10\% higher than the data for CMASS, and within 1\% for GAMA.

%The LOWZ mocks is have b= 1.8, which translates into a clustering about 20% lower than the data. Adjust for this in the error bars by inflating the w(theta) measurements by  (b_data/1.8)^2. This clustering matches the linear bias predictions for 7' < theta < 60'. Below, bias is non-linear, above, finite box effects kick in. We can correct for this. 

%The CMASS mocks is have b= 2.1, which translates into a clustering about 20% higher than the data. Adjust for this in the error bars by deflating the w(theta) measurements by  (b_data/2.1)^2. This clustering matches the linear bias predictions for 1.5' < theta < 60'. Below, bias is non-linear, above, finite box effects kick in. We can correct for this. 

%The GAMA mocks is have b= 1.3, which translates into a clustering about 15% higher than the data. Adjust for this in the error bars by adjusting the w(theta) measurements by  (b_data/1.3)^2. This clustering matches the linear bias predictions for 0.6' < theta < 150'. Below, bias is non-linear, above, finite box effects kick in. We can correct for this. 





